Inverse problems for a quasilinear strongly damped wave equation arising in nonlinear acoustics

We consider inverse problems for a Westervelt equation with a strong damping and a time-dependent potential $q$. We first prove that all boundary measurements, including the initial data, final data, and the lateral boundary measurements, uniquely determine $q$ and the nonlinear coefficient $\beta$. The proof is based on complex geometric optics construction and the approach proposed by Isakov. Further, by considering fundamental solutions supported in a half-space constructed by H\"ormander, we prove that with vanishing initial conditions the Dirichlet-to-Neumann map determines $q$ and $\beta$.

==> newGOC_grow.tex <==
\section{Recovery from the DN map}\label{sec_gocnew}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we would like to improve the results in Section \ref{sec_allbd} using fundamental solutions constructed for the characteristic Cauchy problem, see Section \ref{subsec_cauchy}.
We prove the recovery of $q, \beta$ from the lateral boundary  measurements.
\subsection{The reminder term}\label{subsec_reminder_new}
We reconsider the approximate solution constructed for the linear problem.
The aim is to construct a reminder term $r_N$ satisfying
\[
\opq(v + e^{i\varphi} r_N) = 0 \qquad \text{in }(0, T) \times \Omega
\]
with $r_N$ relatively small,
as well as, with the zero initial conditions.
Recall
we write $P = \partial^2_t - \Delta - \partial_t\Delta$.
%Its symbol is given by
%\[
%P(\tau, \xi) = -\tau^2 + \xi \cdot \xi + i\tau \xi \cdot \xi, \quad \text{for }(\tau, \xi) \in \mathbb{R} \times \mathbb{R}^n.
%\]
%For a multi-index $\alpha = (\alpha_0, \alpha_1, \ldots, \alpha_n)$,
%recall we write
%\[
%P^{(\alpha)}(\tau, \xi) = \partial^\alpha P(\tau, \xi), \qquad
%\tP(\tau, \xi) = (\sum_{\alpha \geq 0} |P^{(\alpha)}(\tau, \xi) |^2)^{1/2}.
%\]
%Then a direct computation shows that
%\begin{align}\label{eq_tPgeq_new}
%\tP^2(\tau, \xi) \geq
%%|-\tau^2 + \xi \cdot \xi + i\tau \xi \cdot \xi|^2 +
% |2 (1 + i\tau) \xi |^2.
%\end{align}
Now we prove the following proposition about the reminder term.
\begin{pp}\label{pp_reminder_new}
    %Suppose $q \in C^\qCm([0,T] \times \bar{\Omega})$.
    For $N \geq 0$, a large parameter $\rho$, and $\omega \in \mathbb{S}^{n-1}$, let $v
    _N(t,x)$ be the approximate solution constructed in (\ref{eq_vN}),
    with the phase function $\varphi = -i \rho^2 t + i\rho(x \cdot \omega)$ and the smooth amplitude  $a =  \sum_{j=0}^N\rho^{-j}{a_j(t,x, \omega)}$,
    where $a_0$ is given by (\ref{eq_a0})
    and satisfies  (\ref{transport_1}, \ref{transport_2},
    \ref{transport_j}) for $j = 1, \ldots, N$.
    Then there exists a solution $r_N$ to the equation
    \begin{align}\label{eq_rN_new}
    (P+q)(e^{i \varphi} r_N) = -(P+q) v_N
    \qquad \text{in }(0, T) \times \Omega
    \end{align}
    {with $r_N(0,x) = \partial_t r_N(0, x) = 0$},
    such that for $s \geq 0$, we have
    \[
    \|r_N\|_{H^s((0,T)\times \Omega)} \leq {C_N}{\rho^{-N-1}}, %\|F_N\|_{H^s((0,T)\times \Omega)},
    \]
    where $C_N$ depends on $q, n, \Omega$ and the choice of $\phi, \chi$.
    %({\color{teal} remove this by assuming properties of these cutoff?})
\end{pp}
\begin{proof}
We would like to show the reminder term $r_N$ is relatively small for large $\rho$ and additionally it is supported in $t \geq \vep$ for some small number $\vep > 0$. This implies it satisfies vanishing initial conditions at $t = 0$.
For this purpose, we recall some conclusions in Section \ref{subsec_cauchy} and modify the notations there for our model.
In the following, let
\begin{align*}
N = (1, 0, \ldots, 0) \in \mathbb{R} \times \Rn, \qquad H = \{(t,x): (t,x) \cdot N \geq \vep\}.
\end{align*}
Note that here we translate the half space by a parameter $\vep$ independent of $\rho$ and it does not affect the estimate in Proposition \ref{pp_Eestimate_new}.
As before, we rewrite (\ref{eq_rN_new}) using $\zetaz = (-i\rho, i\rho \omega)$ to have
\[
(P+q)(e^{i \varphi } r_N)
%= e^{i \varphi} (\sum_\alpha
%\frac{1}{\alpha!}P^{(\alpha)}(\zetaz)  D^\alpha r_0 + q r_0)
= e^{i \varphi} (P(D + \zetaz) r_N + q r_N)
= e^{i \varphi} (\Po r_N + q r_N).
\]
%For convenience, we write $\Po(D) = P(D + \zeta^0)$.
Equation (\ref{eq_rN_new}) can be written as
\begin{align}\label{eq_wR_new}
   P_o(D) r_N = -(\rho^{-N+2} F_N  + q r_N)
\end{align}
where we write $ (P+q) v_N = \rho^{-N+2} e^{i\varphi} F_N$ in (\ref{eq_errorterm}).
Note $ F_N$ is supported in $(0, T) \time \Omega$ with respect to $t$.
Then there exists  $\vep > 0$ such that its support in $t$ is contained in the set of $(\vep, T)$.
Thus, we have $\supp F_N \subset H$.

Note for $P_o(D)$, the boundary $\partial H$ is characteristic, since its principal symbol satisfies $P_{o,3}(N) = 0$.
There is no uniqueness for the initial value problem $P_o(D) u = f$ with $f$ supported in $H$.
As is mentioned before, we would like to find a solution supported in $H$ with the desired estimate, using Proposition \ref{pp_Eestimate_new}.
For this purpose, we prove in Lemma \ref{lm_A1A2} that for our operator $P_o$, there exist $A_1, A_2$ independent of $\rho$ such that condition (\refb) is satisfied.
With this lemma, we set $A_1 = 1$ and $A_2 = 0$. Thus,
we have $P_o(D)$ satisfies (\refb) with $A_1 = A_2 + 1$, which is independent of $\rho$.

Now let $X = (0, T) \times \Omega$ and $\tX$ be a small open neighborhood of $X$.
Let $X_0$ be a small open neighborhood of $\tX- \tX$, which is bounded in $\Rn$.
%Note that $X \subset \{(t,x): |x| \leq \mathrm{diam}(\Omega)\}$.
Then we choose $E_H$ as the bounded linear operator in Proposition \ref{pp_Eestimate_new} for $\Po(D)$ with $X, \tX, X_0$.
For every $r \in H^s(\tX)$ with $\supp r \subset H$,
we consider the map $\mJ(r) = -E_H(\rho^{-N+2}F_N + q r)$,
which has support in $H$ and satisfies
\[
P_o(D)\mJ(r) = - (\rho^{-N+2}F_N + q r) \quad \text{in } X,
\]
with the estimate
\[
\| \mJ(r)\|_{H^s(\tX)} \leq C  \sup_{\zeta \in \mathbb{R}^{n+1}} \frac{1}{\tP_o(\zeta)} \|\rho^{-N+2}F_N + q r\|_{H^s(\tX)},
\]
where $C$ is independent of $\rho$.
On the other hand, we compute
\begin{align*}
    \tP_o^2(\zeta) = \tP^2(\zeta + \zetaz)
    \geq |2(1 + i(\tau - i\rho^2))(\xi + i\rho \eta)|^2
    = 4((1 + \rho^2)^2 + \tau^2)(|\xi|^2 + \rho^2)  \geq 4 \rho^6.
\end{align*}
It follows that for any $r \in H^s(\tX)$ supported in $H$, we have
\begin{align}\label{eq_Jw_new}
\| \mJ(r)\|_{H^s(\tX)} \leq  {C}({\rho}^{-N-1} \|F_N\|_{H^s(\tX)}  + \rho^{-3}\|q\|_{C^{\lceil s \rceil}([0,T] \times \bar{\Omega})} \|r\|_{H^s(\tX)}).
\end{align}
where we extend $q\in C^{\infty}(\bar{X})$ to a function in  $C^{\infty}(\tX)$.
This motivates us to define
\[
H^{s,H}(\tX) = \{u: u \in H^s(\tX) \text{ with $\supp u \subset H$}\}.
\]
%Note that $F_0 \in H^{s,H}(X)$.
%We have $\mJ r \in H^{s,H}(X)$ with
%\[
%\|\mJ (r)\|_{H^s(X)} \leq {C}{\rho}^{-1}\| F_0 + qr\|_{H^s(X)}
%\]
If we choose  $\rho$ large enough such that $ \rho > \max\{2C\|q\|_{C^{\lceil s \rceil}([0,T] \times \bar{\Omega})} , 2CC_{F_0}\}$, then we have
\[
\|\mJ (r)\|_{H^s(\tX)} \leq (1+  \|r\|_{H^s(\tX)})/2 \leq 1,
\]
for any $\|r\|_{H^s(\tX)} \leq 1$.
Thus, the operator $\mJ$ maps the ball $B_1 = \{r \in H^{s,H}(\tX): \|r\|_{H^{s}(\tX)} \leq 1\}$ to itself.
Next, we prove $\mJ$ is a contraction for large $\rho$.
Indeed, for $r_1, r_2 \in H^s(\tX)$,
we compute
\begin{align*}
    \|\mJ(r_2) - \mJ(r_1)\|_{H^s(\tX)}
    = & \|E_H(q(r_2 - r_1))\|_{H^s(\tX)} \\
    \leq & \rho^{-3} C \|q\|_{C^{\lceil s \rceil}([0,T] \times \bar{\Omega})}  \|r_2 - r_1\|_{H^s(\tX)}
    < \frac{1}{2}\|r_2 - r_1\|_{H^s(\tX)}.
\end{align*}
Then by Banach's contraction theorem, there is a function $r_N$ in $B_1$ satisfying $r_N = \mJ(r_N)$, which solves
(\ref{eq_rN_new}).
Note that $r_N$ satisfies the inequality (\ref{eq_Jw_new}), and therefore we have
\[
\frac{1}{2}\|r_N\|_{H^s(\tX)} =
\|\mathcal{J}(r_N)\|_{H^s(\tX)} -  \frac{1}{2}\|r_N\|_{H^s(\tX)}
\leq  C \rho^{-N-1}\|F_N\|_{H^s(\tX)}.
\]
In particular, this implies $\|r_N\|_{H^s(X)} \leq  C_N \rho^{-N-1}\|F_N\|_{H^s(\tX)},$ for some constant $C_N$ independent of $\rho$.
%depending on $q, n, \Omega$ and the choice of $\phi, \chi$.
\end{proof}

\begin{lm}\label{lm_A1A2}
    Let $P$, $\zeta_0$, $N$ be defined as above.
    Suppose $\sigma(\zeta)$ is a solution to $\Po(\zeta + \sigma N)$, where $\zeta = (\tau, \xi) \in \mathbb{C} \times \mathbb{C}^n$.
    If $\sigma(\zeta)$ is analytic and single-valued in a ball $B \subset \mathbb{C} \times \mathbb{C}^n$ with real center and radius $A_1 = 1$,
    then we have
    \[
    \sup_{\zeta \in B} \mathrm{Im} (\sigma(\zeta)) \geq 0.
    \]
\end{lm}
\begin{proof}
    First, we would like to solve $\tau(\xi)$ from $P(\tau, \xi) = 0$ for $\xi \in \mathbb{C}^n$.
    %Then we must have $\sigma(\tau, \xi) = \tau(\xi + \rho \eta) - \tau$.
    Indeed, the equation $-\tau^2 + i \tau \xi \cdot \xi + \xi \cdot \xi = 0$ have two complex roots
    \begin{align*}
        \tau_\pm(\xi)
        %= \frac{1}{2}(i\xi \cdot \xi  \pm \sqrt{-(\xi \cdot \xi)^2 + 4 \xi \cdot \xi}).
        = \frac{1}{2}(iR(\xi)  \pm \sqrt{-R^2(\xi) + 4 R (\xi)}),
        \qquad \text{where }R(\xi) = \xi \cdot \xi.
        %    \qquad
        %    \tau_2 = \frac{1}{2}(i\xi \cdot \xi ) - \sqrt{-(\xi \cdot \xi)^2 + 4 \xi \cdot \xi}.
    \end{align*}
%    In the following, we write
%    \[
%    R(\xi) = \xi \cdot \xi, \qquad
%    \triangle(\xi) = {-R^2(\xi) + 4 R(\xi)}.
%    \]
    Recall $\zetaz = (-i \rho^2, i \rho \omega)$.
    Then the roots for $P_o(\zeta + \sigma N)  = P(\zeta + \zeta^0 + \sigma N) = 0$ are given by
    \begin{align*}
        \sigma_\pm(\tau, \xi) &= \frac{1}{2}(iR(\xi + i \rho \omega)
        \pm \sqrt{\triangle(\xi + i \rho \omega)})  + i\rho^2 - \tau.
    \end{align*}
    For a ball $B$ centered at $(\tau, \xi)\in \mathbb{R} \times \Rn$,
    we write $(\tau, \xi) = (0, r \theta)$, where $r \geq 1$ and $\theta \in \mathbb{S}^{n-1}$.
    First we compute
    \[
    R(\xi + i \rho \omega) = (r^2 - \rho^2) + i 2 r \rho (\omega \cdot \theta)
    \coloneqq c + id,
    \]
    and
    \[
    -R^2(\xi) + 4 R (\xi) = (d^2 - c^2 + 4c) + i 2d(2-c) \coloneqq C + iD,
    \]
    where $c, d, C, D \in \mathbb{R}$.
    Suppose $C + iD = (a + ib)^2$ for some real numbers $a, b$.
    Then a straightforward computation shows that
    \[
    b^2 = \frac{1}{2}(-C + \sqrt{C^2 + D^2}).
    \]
    Note that
    \begin{align*}
    C^2 + D^2 &= (d^2 - c^2 + 4c)^2 + 4d^2(2-c)^2 \\
              & = ((d^2 +4) - (c-2)^2)^2 + 4(d^2+4)(c-2)^2 -16(c-2)^2 \\
              & \leq ((d^2 +4) + (c-2)^2)^2.
    \end{align*}
    This implies that
    \[
    b^2 \leq \frac{1}{2}(-(d^2 - c^2 + 4c) +(d^2 +4) + (c-2)^2) = (c-2)^2.
    \]
    Then we have
    \[
    (c + 2\rho^2)^2 - b^2 \geq (r^2 + \rho^2)^2 - (r^2 - \rho^2 -2)^2  = 4(\rho^2 + 1)(r^2 -1) \geq 0.
    \]
    Note $c +2 \rho^2 = r^2 + \rho^2 \geq 0$.
    Thus, the imaginary part of the roots satisfies
    \[
    \mathrm{Im}(\sigma_\pm(0, r\theta)) = \frac{1}{2}(c + 2\rho^2 \pm b) \geq 0.
    \]
    This proves for any ball $B$ with real center and radius $A_1$, we have
    \[
    \sup_{\zeta \in B} \mathrm{Im} (\sigma(\zeta)) \geq A_2 = 0,
    \]
    if $\sigma(\zeta)$ is a real-valued and analytic root.
%    \newpage
%
%    Note that $\sqrt{z}$ is analytic and single-valued in $\mathbb{C}\setminus\{(-\infty,0]\}$.
%    Then the two roots are analytic and single-valued away from the set
%    \[
%    {\teal \{(\tau, \xi) \in \mathbb{C} \times \mathbb{C}^n: \mathrm{Re}(\triangle(\tau, \xi + \rho \eta))\leq 0 \text{ and } \mathrm{Im}(\triangle(\tau, \xi + \rho \eta)) = 0 \}}.
%    \]
%    For convenience, we write  $R(\xi) = \xi \cdot \xi + 2 \rho \eta \cdot \xi = a_1 + ib_1$, where $a_1,b_1 \in \mathbb{R}$.
%    Then we compute
%    \[
%    \triangle(\tau, \xi + \rho \eta) = -R^2(\xi + \rho\eta) + 4 R(\xi + \rho\eta) =b_1^2 - a_1^2 +4a_1 + i2b_1(2-a_1).
%    \]
%    On the other hand, we write $\xi = \omega_1 + \varsigma_1 + i \varsigma_2$ for $\xi \in B$, where $\varsigma_1, \varsigma_2 \in \Rn$ with $|\varsigma_1|^2 + |\varsigma_2|^2 \leq 1/16$ for $j =1,2$.
%    We compute
%    \begin{align*}
%        R(\xi) = (\omega_1 + \varsigma_1 + i \varsigma_2) \cdot (\omega_1 + \varsigma_1 + i \varsigma_2) + 2 \rho (i \omega_1 + \omega_2) \cdot (\omega_1 + \varsigma_1 + i \varsigma_2)
%    \end{align*}
%    and we have
%    \begin{align*}
%        b_1  = \mathrm{Im}(R(\xi)) =  2 \varsigma_2 \cdot \omega_1 + 2 \varsigma_1 \cdot \varsigma_2
%        + 2 \rho + 2\rho (\omega_1 \cdot \varsigma_1 + \omega_2 \cdot \varsigma_2).
%    \end{align*}
%    Note that we have
%    \[
%    |b_1| \geq 2 \rho  - 2|\varsigma_2 \cdot \omega_1| - 2 |\varsigma_1 \cdot \varsigma_2| - 2\rho |\omega_1 \cdot \varsigma_1 + \omega_2 \cdot \varsigma_2|
%    \geq 2\rho -\frac{1}{4} - \frac{1}{8} - \rho \geq \rho - \frac{3}{8},
%    \]
%    which is nonzero for large $\rho$.
%    When $a_1 = 2$, we have $\mathrm{Re}(\triangle(\tau, \xi + \rho\eta)) > 0$ in $B$.
%    When $a_1 \neq 2$, we have $\mathrm{Im}(\triangle(\tau, \xi + \rho\eta)) \neq 0$ in $B$.
%    Thus, the roots $\sigma_\pm(\tau, \xi)$ are analytic and single-valued there.
%
%    Next, we would like to find an lower bound of $\sup_B \mathrm{Im} (\sigma(\zeta))$.
%    Indeed, note that we have
%    $R(\omega_1) = 1 + 2 i \rho$ and
%    $\triangle(0, \omega_1) = \sqrt{3 + 4 \rho^2 + 4i\rho}$.
%    To find out its imaginary part, we write $3 + 4 \rho^2 + 4i\rho = (a_2 + ib_2)^2$, where $a_2, b_2 \in \mathbb{R}$.
%    A straightforward computation shows that
%    \begin{align*}
%        b_2^2
%        = \frac{1}{2}(-(3 + 4 \rho^2) + \sqrt{(3 + 4 \rho^2)^2 + 16 \rho^2})
%        &=\frac{8\rho^2}{(3 + 4 \rho^2) + \sqrt{(3 + 4 \rho^2)^2 + 16 \rho^2}}\\
%        & = \frac{8}{(\frac{3}{\rho^2} + 4) + \sqrt{(\frac{3}{\rho^2} + 4 )^2 + \frac{16}{\rho^2}}}
%        \leq \frac{1}{2}
%    \end{align*}
%    for large $\rho$.
%    This implies
%    \[
%    \mathrm{Im}(\sigma_\pm(0, \omega_1)) \geq \frac{1}{2} - \frac{\sqrt{2}}{2} \geq -\frac{1}{4}
%    \]
%    and therefore we have $\sup_B \mathrm{Im} (\sigma(\zeta)) \geq -\frac{1}{4}$.
%    This proves the lemma.
\end{proof}

